A Survey on Protein Representation Learning: Retrospect and Prospect

Proteins are fundamental biological entities that play a key role in life activities. The amino acid sequences of proteins can be folded into stable 3D structures in the real physicochemical world, forming a special kind of sequence-structure data. With the development of Artificial Intelligence (AI) techniques, Protein Representation Learning (PRL) has recently emerged as a promising research topic for extracting informative knowledge from massive protein sequences or structures. To pave the way for AI researchers with little bioinformatics background, we present a timely and comprehensive review of PRL formulations and existing PRL methods from the perspective of model architectures, pretext tasks, and downstream applications. We first briefly introduce the motivations for protein representation learning and formulate it in a general and unified framework. Next, we divide existing PRL methods into three main categories: sequence-based, structure-based, and sequence-structure co-modeling. Finally, we discuss some technical challenges and potential directions for improving protein representation learning. The latest advances in PRL methods are summarized in a GitHub repository https://github.com/LirongWu/awesome-protein-representation-learning.

==> PRL Survey/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> PRL Survey/overview.tex <==
\tikzstyle{leaf}=[
draw=hiddendraw,
rounded corners,
minimum height=1.2em,
fill=hidden-orange!40,
text opacity=1, 
align=center,
fill opacity=.5,  
text=black,
align=left,
font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]

\tikzstyle{level0}=[
draw=hiddendraw,
rounded corners,
minimum height=1.2em,
fill=hidden-cy!20,
text opacity=1, 
align=center,
fill opacity=.5,  
text=black,
align=left,
font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]

\tikzstyle{level1}=[
draw=hiddendraw,
rounded corners,
minimum height=1.2em,
fill=hidden-blue!150,
text opacity=1, 
align=center,
fill opacity=.5,  
text=black,
align=left,
font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]

\tikzstyle{level2}=[
draw=hiddendraw,
rounded corners,
minimum height=1.2em,
fill=output-purple,
text opacity=1, 
align=center,
fill opacity=.5,  
text=black,
align=left,
font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]

\tikzstyle{level3}=[
draw=hiddendraw,
rounded corners,
minimum height=1.2em,
fill=output-green!40,
text opacity=1, 
align=center,
fill opacity=.5,  
text=black,
align=left,
font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]


\begin{figure*}[t]
\centering
% \vspace{-2em}
\begin{forest}
  for tree={
  forked edges,
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=middle,
  font=\scriptsize,
  rectangle,
  draw=hiddendraw,
  rounded corners,
  align=left,
  minimum width=2.5em,
  minimum height=1.2em,
    s sep=6pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  where level=1{font=\scriptsize}{},
  where level=2{font=\scriptsize}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [PRL, level0
    [Preliminaries,level1
        [Notation and Problem Statement,level2]
    ]
    [Architectures,level1
        [Sequence-based,level2
            [Single Sequence,level3
                [LSTM \cite{hochreiter1997long}{,}~Transformer \cite{vaswani2017attention}{,}~CNNs \cite{lecun1995convolutional},leaf]
            ]
            [MSA Sequence,level3
                [MSA Transformer \cite{rao2021msa}{,}~Evoformer \cite{jumper2021highly},leaf]
            ]
        ]  
        [Structure-based,level2
            [Feature map-based,level3
                [3D CNNs \cite{derevyanko2018deep}{,}~Spherical CNNs \cite{sverrisson2021fast},leaf]
            ]
            [Message-passing GNNs,level3
                [GCNs \cite{kipf2016semi}{,}~IEConv \cite{hermosilla2020intrinsic}{,}~GearNet \cite{zhang2022protein},leaf]
            ]
            [Geometric GNNs,level3
                [GVP \cite{jing2020learning}{,}~GBP \cite{aykent2022gbpnet}{,}~DWP \cite{li2022directed},leaf]
            ]
        ]  
        [Sequence-structure Co-modeling,level2
            [DeepFRI \cite{gligorijevic2021structure}{,}~LM-GVP \cite{wang2021lm},leaf]
        ]  
    ]
    [Pretext Tasks,level1
        [Sequence-based,level2
            [Supervised,level3
                [PLUS \cite{min2021pre}{,}~Profile Prediction \cite{sturmfels2020profile}{,}~Progen \cite{madani2020progen},leaf]
            ]
            [Self-Supervised,level3
                [MLM \cite{rao2019evaluating}{,}~PMLM \cite{he2021pre}{,}~NAP \cite{alley2019unified}{,}~CPC \cite{lu2020self},leaf]
            ]
        ]  
        [Structure-based,level2
            [Contrative,level3
                [Multiview Contrast \cite{hermosilla2022contrastive,zhang2022protein},leaf]
            ]
            [Predictive,level3
                [Distance and Angle Prediction \cite{chen2022structure}{,}~Dihedral Prediction \cite{hermosilla2022contrastive},leaf]
            ]
        ]  
        [Sequence-structure Co-modeling,level2
            [Full-atomic Structure Prediction \cite{jumper2021highly,hu2022exploring},leaf]
        ]  
    ]
    [Applications,level1
        [Property Prediction,level2
            [Stability \cite{rao2019evaluating}{,}~Fold Quality \cite{baldassarre2021graphqa}{,}~Mutation Effect \cite{meier2021language}{,}~PPI \cite{wang2019high},leaf]
        ]  
        [Structure Prediction,level2
            [Full-atomic or Backbone Prediction \cite{hiranuma2021improved,wu2022high}{,}~Structure Inpainting \cite{mcpartlon2022attnpacker},leaf]
        ]  
        [Protein Design,level2
            [Template-based \cite{ingraham2019generative}{,}~De Novo \cite{huang2016coming,koepnick2019novo},leaf]
        ]  
        [Structure-Based Drug Design,level2
            [Auto-regressive \cite{liu2022graphbp,peng2022pocket2mol}{,}~Diffusion \cite{lin2022diffbp,schneuing2022structure},leaf]
        ]  
    ]
  ]
\end{forest}
\caption{A high-level overview of this survey with representative examples.}
% \vspace{-1em}
\label{fig:2}
\end{figure*}

==> PRL Survey/table_1.tex <==
\begin{table*}[!tbp]
\begin{center}
% \vspace{-1.5em}
\caption{Summary of representative protein representation learning methods.}
\label{tab:1}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccl}

\toprule
\textbf{Method} & \textbf{Category} & \textbf{Architecture} & \textbf{Pretext Task} & \textbf{Year} \\ \midrule
Bio2Vec-CNN \cite{wang2019high} & \cellcolor{gray!20}Sequence-based & CNN & - & 2019 \\ \hline
TAPE \cite{rao2019evaluating} & \cellcolor{gray!20}Sequence-based & ResNet, LSTM, Transformer & \tabincell{c}{Masked Language Modeling, \\ Next Amino Acid Prediction} & 2019 \\ \hline
UniRep \cite{alley2019unified} & \cellcolor{gray!20}Sequence-based & Multiplicative LSTM & Next Amino Acid Prediction & 2019 \\ \hline
TripletProt \cite{nourani2020tripletprot} & \cellcolor{gray!20}Sequence-based & Siamese Networks & Contrastive Predictive Coding & 2020 \\ \hline
PLP-CNN \cite{shanehsazzadeh2020transfer} & \cellcolor{gray!20}Sequence-based & CNN & - & 2020 \\ \hline
CPCProt \cite{lu2020self} & \cellcolor{gray!20}Sequence-based & GRU, LSTM & Contrastive Predictive Coding & 2020 \\ \hline
MuPIPR \cite{zhou2020mutation} & \cellcolor{gray!20}Sequence-based & GRU, LSTM & Next Amino Acid Prediction & 2020 \\ \hline
ProtTrans \cite{elnaggar2020prottrans} & \cellcolor{gray!20}Sequence-based & Transformer, Bert, XLNet & Masked Language Modeling  & 2020 \\ \hline
DMPfold \cite{kandathil2020deep} & \cellcolor{gray!20}Sequence-based & GRU, ResNet & - & 2020 \\ \hline
Profile Prediction \cite{sturmfels2020profile} & \cellcolor{gray!20}Sequence-based & Transformer & HMM Profile Prediction  & 2020 \\ \hline
PRoBERTa \cite{nambiar2020transforming} & \cellcolor{gray!20}Sequence-based & Transformer & Masked Language Modeling & 2020 \\ \hline
UDSMProt \cite{strodthoff2020udsmprot} & \cellcolor{gray!20}Sequence-based & LSTM & Next Amino Acid Prediction & 2020 \\ \hline
ESM-1b \cite{rives2021biological} & \cellcolor{gray!20}Sequence-based & Transformer & Masked Language Modeling & 2021 \\ \hline
PMLM \cite{he2021pre} & \cellcolor{gray!20}Sequence-based & Transformer & Pairwise Masked Language Modeling & 2021 \\ \hline
MSA Transformer \cite{rao2021msa} & \cellcolor{gray!20}Sequence-based & MSA Transformer & Masked Language Modeling & 2021 \\ \hline
ProteinLM \cite{xiao2021modeling} & \cellcolor{gray!20}Sequence-based & BERT & Masked Language Modeling & 2021 \\ \hline
PLUS \cite{min2021pre} & \cellcolor{gray!20}Sequence-based & Bidirectional RNN & \tabincell{c}{Masked Language Modeling, \\ Same-Family Prediction} & 2021  \\ \hline
Adversarial MLM \cite{mcdermott2021adversarial} & \cellcolor{gray!20}Sequence-based & Transformer & \tabincell{c}{Masked Language Modeling, \\ Adversarial Training} & 2021  \\ \hline
ProteinBERT \cite{brandes2022proteinbert} & \cellcolor{gray!20}Sequence-based & BERT & Masked Language Modeling & 2022 \\ \hline
CARP \cite{yang2022convolutions} & \cellcolor{gray!20}Sequence-based & CNN & Masked Language Modeling & 2022  \\

\midrule \midrule
3DCNN \cite{derevyanko2018deep} & \cellcolor{red!20}Structure-based & 3DCNN & - & 2018 \\ \hline
IEConv \cite{hermosilla2020intrinsic} & \cellcolor{red!20}Structure-based & IEConv & - & 2020 \\ \hline
GVP-GNN \cite{jing2020learning} & \cellcolor{red!20}Structure-based & GVP & - & 2020 \\ \hline
GraphMS \cite{cheng2021graphms} & \cellcolor{red!20}Structure-based & GCN & Multiview Contrast & 2021 \\ \hline
DL-MSFM \cite{gelman2021neural} & \cellcolor{red!20}Structure-based & GCN & - & 2021 \\ \hline
PG-GNN \cite{xia2021geometric} & \cellcolor{red!20}Structure-based & PG-GNN & - & 2021 \\ \hline
CRL \cite{hermosilla2022contrastive} & \cellcolor{red!20}Structure-based & IEConv & Multiview Contrast & 2022 \\ \hline
DW-GNN \cite{li2022directed} & \cellcolor{red!20}Structure-based & DWP & - & 2022 \\ \hline
GBPNet \cite{aykent2022gbpnet} & \cellcolor{red!20}Structure-based & GBP & - & 2022 \\ \hline
GearNet \cite{zhang2022protein} & \cellcolor{red!20}Structure-based & GearNet & \tabincell{c}{Multiview Contrast, \\ Distance and Dihedral Prediction,  \\ Residue Type Prediction} & 2022 \\ \hline
ATOMRefine \cite{wu2022atomic} & \cellcolor{red!20}Structure-based & SE(3) Transformer & - & 2022 \\ \hline
STEPS \cite{chen2022structure} & \cellcolor{red!20}Structure-based & GIN & Distance and Dihedral Prediction & 2022 \\


 \midrule \midrule
GraphCPI \cite{quan2019graphcpi} & \cellcolor{blue!20}Co-Modeling & CNN, GNN &  - & 2019 \\ \hline
MT-LSTM \cite{bepler2019learning} & \cellcolor{blue!20}Co-Modeling & Bidirectional LSTM &  \tabincell{c}{Contact prediction, \\ Pairwise Similarity Prediction} & 2019 \\ \hline
LM-GVP \cite{wang2021lm} & \cellcolor{blue!20}Co-Modeling & Transformer, GVP & - & 2021 \\ \hline
AlphaFold2 \cite{jumper2021highly} & \cellcolor{blue!20}Co-Modeling & Evoformer &  \tabincell{c}{Masked Language Modeling, \\ Full-atomic Structure Prediction} & 2021 \\ \hline
DeepFRI \cite{gligorijevic2021structure} & \cellcolor{blue!20}Co-Modeling & LSTM, GCN & - & 2021 \\ \hline
HJRSS \cite{mansoor2021toward} & \cellcolor{blue!20}Co-Modeling & SE(3) Transformer &  \tabincell{c}{Masked Language Modeling, \\ Graph Completion} & 2021 \\ \hline
GraSR \cite{xia2022fast} & \cellcolor{blue!20}Co-Modeling & LSTM, GCN & Momentum Contrast & 2022 \\ \hline
CPAC \cite{you2022cross} & \cellcolor{blue!20}Co-Modeling & Hierarchical RNN, GAT & \tabincell{c}{Masked Language Modeling, \\ Graph Completion} & 2022 \\ \hline
MIF-ST \cite{yang2022masked} & \cellcolor{blue!20}Co-Modeling & CNN, GNN & Masked Inverse Folding & 2022 \\ \hline
OmegaFold \cite{wu2022high} & \cellcolor{blue!20}Co-Modeling & Geoformer & \tabincell{c}{Masked Language Modeling, \\ Full-atomic Structure Prediction} & 2022 \\
 \bottomrule
 
\end{tabular}} \vspace{-0.6em}
\end{center}
\end{table*}
